Diagrammatic Negative Information

The flow of information through a complex system can be readily understood with category theory. However, negative information (e.g., what is not possible) does not have an immediately evident categorical representation. The formalization of nategories using unconventional composition addresses this issue, and lets imposed limitations on categories be considered. However, traditional nategories abandon core categorical constructs and rely on extensive mathematical development. This creates a divide between the consideration of positive and negative information composition. In this work, we show that negative information can be considered in a natural categorical manner. This is aided by functor string diagrams, a novel flexible diagrammatic approach that can intuitively show the operation of hom-functors and natural transformations in expressions. This insight reveals how to consider the composition of negative information with foundational categorical constructs without relying on enrichment. We present diagrammatic means to consider not only nategories, but preorders more broadly. This paper introduces diagrammatic methods for the consideration of triangle inequalities and co-designs $\mathbf{DP/Feas_{Bool}}$, showing how important cases of negative information composition can be categorically and diagrammatically approached. In particular, we develop systematic tools to rigorously consider imposed limitations on systems, advancing our mathematical understanding, and present intuitive diagrams which motivate widespread adoption and usage for various applications.

==> utils/other-symbols.tex <==
%
%
%
\newcommand{\prf}{\expandafter\prftree[r]{\raisebox{3pt}{}}}
\newcommand{\prfdouble}{\expandafter\prftree[double]}
\newcommand{\prfcomma}{\expandafter\prftree[r]{\raisebox{3pt}{,}}}
\newcommand{\prfperiod}{\expandafter\prftree[r]{\raisebox{3pt}{.}}}
\newcommand{\prfsemi}{\expandafter\prftree[r]{\raisebox{3pt}{;}}}
\newcommand{\prfdoublecomma}{\expandafter\prftree[double][r]{\raisebox{3pt}{,}}}
\newcommand{\prfdoubleperiod}{\expandafter\prftree[double][r]{\raisebox{3pt}{.}}}


\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother


\newcommand{\gear}[5]{%
\begin{tikzpicture}
\draw[ultra thick]
\foreach \i in {1,...,#1} {%
  [rotate=(\i-1)*360/#1]  (0:#2)  arc (0:#4:#2) {[rounded corners=1.5pt]
             -- (#4+#5:#3)  arc (#4+#5:360/#1-#5:#3)} --  (360/#1:#2)
};\end{tikzpicture}}

%
%
%
%


\newcommand{\sectionexercises}[1]{%
    \section[Code exercises - #1]{\texorpdfstring{\usebox{\chaptergear}}{Code exercises -} #1}
}

%

\newcommand{\RposgenBel}{\R{\posgenBel}}
\newcommand{\FposgenAel}{\F{\posgenAel}}
\newcommand{\FposgenBel}{\F{\posgenBel}}
\newcommand{\FposgenAelop}{\F{\posgenAel^*}\!\!}
\newcommand{\FposgenBelop}{\F{\posgenBel^*}\!\!}
\newcommand{\FposgenCelop}{\F{\posgenCel^*}\!\!}

\newcommand{\lens}[6]{\begin{pmatrix} #1\\ #4\end{pmatrix}\colon \begin{pmatrix} #2\\ #5\end{pmatrix} \leftrightarrows \begin{pmatrix} #3\\ #6\end{pmatrix}}
\newcommand{\lensa}{\lens{\pbacka}{\setlensam}{\setlensbm}{\pforwa}{\setlensap}{\setlensbp}}
\newcommand{\lensb}{\lens{\pbackb}{\setlensbm}{\setlenscm}{\pforwb}{\setlensbp}{\setlenscp}}
\newcommand{\lenscd}{\lens{\pbackb}{\setlenscm}{\setlensdm}{\pforwb}{\setlenscp}{\setlensdp}}
\newcommand{\lensinterf}[2]{\begin{pmatrix}#1 \\ #2\end{pmatrix}}

\newcommand{\funcnameT}[1]{\funcnamestyle{#1()}\xspace}

\newcommand{\funcname}[1]{\funcnamestyle{\detokenize{#1}()}\xspace}
%
\newcommand{\fieldname}[1]{\fieldnamestyle{#1}\xspace} %
%
\newcommand{\classname}[1]{\classnamestyle{#1}\xspace} %
%



\DeclareMathSymbol{\shortminus}{\mathbin}{AMSa}{"39}
\newcommand{\shortplus}{{{+}}} %
\newcommand{\minusone}{{{\shortminus}}\kern1pt1}
\newcommand{\plusone}{\shortplus1}


\makeatletter
\DeclareRobustCommand{\shortto}{%
    \mathrel{\mathpalette\short@to\relax}%
}

\newcommand{\short@to}[2]{%
    \mkern2mu
    \clipbox{{.4\width} 0 0 0}{$\m@th#1\vphantom{+}{\shortrightarrow}$}%
}
\makeatother


\makeatletter



\newcommand{\opensetbracket}{{\ColorIfNowBlack{formulasetcolor}{\mathbf{\{}}}}
\newcommand{\closesetbracket}{{\ColorIfNowBlack{formulasetcolor}{\mathbf{\}}}}}

%
%


\newcommand{\cleft}[2][.]{%
    \begingroup\colorlet{savedleftcolor}{.}%
    \color{#1}\mathopen{}\left#2\color{savedleftcolor}%
}
\newcommand{\cright}[2][.]{%
    \color{#1}\right#2\mathclose{}\endgroup%
}



\DeclareRobustCommand{\@makelists}[4]{%
    #1%
    \foreach \entry [count=\xi]  in {#4}{
        \ifnum\xi = 1\else#2\linebreak[0]\fi%
        {{\entry}}%
    }%
    #3%
}
\newcommand{\smallspace}{\mspace{4mu}}
\newcommand{\commaspace}{{,\smallspace}}
\DeclareRobustCommand{\makeset}[1]{%
    \@makelists{\opensetbracket}{\commaspace}{\closesetbracket}{#1}%
}
\DeclareRobustCommand{\makesetnocolor}[1]{%
    \@makelists{\{}{\commaspace}{\}}{#1}%
}
\DeclareRobustCommand{\tupp}[1]{%
    \@makelists{\langle}{\commaspace}{\rangle}{#1}%
}

%
%

\DeclareRobustCommand{\tup}[1]{%
        \@makelists{\mathopen{}\left\langle}{\commaspace}{\right\rangle\mathclose{}}{#1}%
}

\DeclareRobustCommand{\makecprod}[1]{%
    \@makelists{}{\cprod}{}{#1}%
}

\DeclareRobustCommand{\makecartprod}[1]{%
    \@makelists{}{\cartprod}{}{#1}%
}

\DeclareRobustCommand{\maketupconcat}[1]{%
    \@makelists{}{\tupconcat}{}{#1}%
}

\DeclareRobustCommand{\maketypedlist}[2]{%
    \makelist{#1}_{#2}%
}

\DeclareRobustCommand{\makesetBig}[1]{%
    \@makelists{{\mathopen{}\color{formulasetcolor}\mathbf{\Big\{}}}{\commaspace}{{\color{formulasetcolor}\mathbf{\Big\}}\mathclose{}}}{#1}%
}

\DeclareRobustCommand{\makesett}[1]{%
    \@makelists{\cleft[formulasetcolor]{\{}}{\commaspace}{\cright[formulasetcolor]{\}}}{#1}%
}

\DeclareRobustCommand{\makelist}[1]{%
    \@makelists{[}{\commaspace}{]}{#1}%
}

\DeclareRobustCommand{\cObj}[1]{%
    \@makelists{\fatstart}{\commaspace}{\fatend}{#1}%
}

%
\makeatother

\newcommand{\elprime}{\styleelements{'}}


\newcommand{\currydish}{\text{curry}}
\newcommand{\casserole}{\text{casserole}}
\newcommand{\beef}{\text{beef}}
\newcommand{\chicken}{\text{chicken}}

\newcommand{\alphubel}{\textcolor{violet}{ALPHUBEL}}
\newcommand{\bernina}{\textcolor{blue}{BERNINA}}
\newcommand{\someday}{\textcolor{black}{SOMEDAY}}
\DeclarePairedDelimiter\mypars{\lparen}{\rparen}
\newcommand{\pars}[1]{\mypars*{#1}}
\newcommand{\parsL}[1]{\Big(#1\Big)}
\newcommand{\parslight}[1]{\cleft[lightgray]{(}#1\cright[lightgray]{)}}


\edef\BlackColor{\csname\string\color@.\endcsname}

\makeatletter
\newcommand{\@CurrentColor}{}%
\DeclareRobustCommand{\ColorIfNowBlack}[2]{%
    \edef\@CurrentColor{\csname\string\color@.\endcsname}%
    \IfStrEq{\@CurrentColor}{\BlackColor}{%
        {\color{#1}#2}%
    }{%
        #2%
    }%
}
\makeatother

%
\newcommand{\raisebigsymbol}[1]{#1} %
%
%
%
%
\newcommand{\boldplus}{\mathbin{\textbf{+}}}
\newcommand{\boldtimes}{\mathbin{\textbf{Ã—}}}
\newcommand{\raisedtextplus}{\mathbin{\textbf{+}}}
\newcommand{\raisedtexttimes}{\mathbin{\textbf{Ã—}}}
\newcommand{\rrangleSAFE}{\texorpdfstring{\rrangle}{<<}}
\newcommand{\llangleSAFE}{\texorpdfstring{\llangle}{>>}}


==> utils/packages-act.tex <==
\usepackage[english]{babel} %

%
%
%
%

%

%

%

%
%
%
%

%
\usepackage[usenames,dvipsnames,table]{xcolor}
%

%

%
%
%
%
%

%
%

%

%
%
%
%

%

\renewcommand{\thepart}{\Alph{part}}

%

%
\newcommand{\outsnippet}[3]{
    \UseVerbatim{#1}
}

%
%
%
%
%

\usepackage{ifthen}
\usepackage{iftex}
\usepackage{ifxetex}
\usepackage[utf8]{inputenc}
%
%
%
%
\usepackage[style=russian]{csquotes}

%

\usepackage{blkarray, array}

\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{xspace}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb} %
\usepackage{mathtools}

%

\usepackage{multirow}
\usepackage{prftree}

%
%
%
%
\usepackage{comment}
\usepackage{accents}

\usepackage{ebproof}
\usepackage{units}

\usepackage{todonotes}
%
%
%

\usepackage{pgfplots}
\pgfplotsset{compat=1.16}
%
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{graphicx}
\usepackage{calc}

\usepackage{adjustbox}
%
\usepackage[section]{placeins}
\usepackage{eso-pic}
\usepackage{capt-of}
\usepackage{wrapfig}
\usepackage[normalem]{ulem}
%
%

%
%
%
%
%
%
%
\usepackage{stmaryrd}
\usepackage{pifont}
%
\usepackage{relsize}

\usepackage{makeidx}

\usepackage{longtable}

\usepackage{multicol}

%
\usepackage{transparent}
\usepackage{datetime2}
\usepackage{anyfontsize}
\usepackage{ifmtarg}

\let\BreakableUnderscore\relax
\usepackage{underscore}


%
\graphicspath{
    {\rootdir/figures/},
    {\rootdir/pics/},
    {\rootdir/slides/},
    {\rootdir/videos/generated/},
    {\rootdir/figures/reits/},
    {\rootdir/figures/firstpaper/},
    {\rootdir/figures/uncertainty/},
    {\rootdir/papers/uncertainty/},
    {},
    {../}}
%
%

%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%

%

%
%
%
%

\newcommand{\pointsize}{0.06}

\newboolean{statuscolors}
\newboolean{instructors}
\newboolean{showslides} %
\newboolean{showproofs}
\newboolean{debugimages}
\newboolean{cachepdf}
\newboolean{devel} %

\newboolean{codeexercises}
\newboolean{githublink}


\newcommand{\instructors}[1]{\ifbool{instructors}{%
        %
        #1
        %
        %
        %
        %
    }{}}

\newcommand{\showslides}[1]{\ifbool{showslides}{#1}{}}

\newcommand{\showproofs}[1]{\ifbool{showproofs}{#1}{}}
\newcommand{\devel}[1]{\ifbool{devel}{%
        \clearpage
        \pagecolor{yellow!7}
        #1
        \clearpage
        \pagecolor{white}
    }{}
}
\newcommand{\toexclude}[1]{\ifbool{devel}{%
        \clearpage
        \pagecolor{gray}
        %
        #1
        %
        %
        \clearpage
        \pagecolor{white}
    }{}
}

%
%
%
%
%

\newcommand{\codeexercises}[1]{%
    \ifbool{codeexercises}{%
        \FloatBarrier
        \clearpage
        \pagecolor{blue!7}
        %
        #1
        %
        %
        \clearpage
        \pagecolor{white}
    }{}%
}

%

\newcommand*{\vcenteredhbox}[1]{\begingroup
    \setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}

\newcommand{\captionsideleft}[2]{
    \medskip
    \begin{minipage}{1.8cm}{
            \hfill
            \protect\captionof{figure}{#1}}\end{minipage}
    \begin{minipage}{6.6cm}
        \vcenteredhbox{{#2}}
        \hfill
    \end{minipage}
    \medskip
}


%

%
%
%
%
%
%
%
%
%
%
\newcommand{\partfirstb}[4]{
    \part{#1}%
    \ifemptyarg{#3}{
        \PackageError{ACT4E}{Empty label argument}{You passed empty label}%
    }{
        \label{#3}%
    }
    \begin{tikzpicture}
        [remember picture,overlay,shift={(current page.north east)}]
        \node[anchor=north east,xshift=5mm,yshift=-3.4cm]{
            \includegraphics[width=\paperwidth+5mm,keepaspectratio=true]{#2.cropped}%
        };
    \end{tikzpicture}
    \vspace{12.4cm}
    #4
    \etocsettocstyle{\rule{\linewidth}{\tocrulewidth}\vskip0.2\baselineskip}{\rule{\linewidth}{\tocrulewidth}}
    \etocsetnexttocdepth{chapter}
    \vfill
    \begin{widepar}
        \localtableofcontents
    \end{widepar}
    \vfill
    \begin{widepar}
        \footnotesize
        \input{\rootdir/pics/#2.tex}
    \end{widepar}
}

\newcommand{\tableColors}{\rowcolors{2}{green!4}{blue!4}}
\newcommand{\tableColorsTwo}{\rowcolors{3}{green!4}{blue!4}}

\newlength{\dpiconwidth}
\setlength{\dpiconwidth}{1.1cm}


\newcommand{\nomencsectionname}[1]{\rule{0pt}{4mm}\textbf{#1}}
\newcommand{\nomencsubsectionname}[1]{\rule{0pt}{4mm}\emph{#1}}
\newcommand{\unused}{{\color{red}unused}~}

%
%

%
%
%
%

%

%
%
%

%

\newcommand{\partended}{
    \cleardoublepage
    \oldsection*{Solutions to selected exercises}
    \printsolutions}

\newenvironment{longcode}{\captionsetup{type=listing,justification=centering}}{}

%
%
%
%
%

%
%
%

%

%
%
%

\newcommand{\punctuate}{
    \todotextjira{381}{@Gioele: punctuate equations}
}

%
%
%
%

%
%
%
%
%

%
%
%
%
%
%
%

%
%
%

%
%
%
%
%
%
%
%
%
%
%


\newcommand{\linkgithub}{
    \ifbool{githublink}{%
        \usebox{\urlbox}%
    }{}
}
\newcommand{\draftnotice}{
    \ifbool{githublink}{%
        \footnotesize You are reading a draft compiled on \DTMnow%
    }{}%
}

%
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%
\let\oldsubseteq\subseteq
\renewcommand{\subseteq}{\mathrel{\oldsubseteq}\linebreak[0]}
\let\oldsupseteq\supseteq
\renewcommand{\supseteq}{\mathrel{\oldsupseteq}\linebreak[0]}
\let\oldsubset\subset
\renewcommand{\subset}{\mathrel{\oldsubset}\linebreak[0]}
\let\oldsupset\supset
\renewcommand{\supset}{\mathrel{\oldsupset}\linebreak[0]}

%
%
%
%

%
\newcommand{\refplus}[1]{\cref{#1} - \nameref{#1}}
%
\newcommand{\chrefplus}[1]{Chapter~\ref{#1} - \nameref{#1}}
\newcommand{\partrefplus}[1]{Part~\ref{#1} - \nameref{#1}}
%
    %
    %
%

%
%
%
%
%

%

%
%

\usepackage{filemod}

\usepackage{trimclip}


%
%
%
%

\usepackage{ulem}
%
%

%
%
%
%
\usepackage{silence}
\WarningsOff[contour]
%

%
%

%
%





==> utils/preamble-act.tex <==
%
%
\usepackage{import}

\input{\rootdir/utils/packages-act}
%
%
\input{\rootdir/utils/tikz-utils}
\input{\rootdir/utils/symbols}
%
\input{\rootdir/utils/symbols-papers}
%
%
%
%
\input{\rootdir/utils/other-symbols}



\newenvironment{forslides}{%
    \colorlet{shadecolor}{Pink!50}%
    \begin{shaded*}%
        \textbf{This content was created for slides. Do not erase or change the names}.\\%
        }{%
    \end{shaded*}}

==> utils/symbols-papers.tex <==
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


==> utils/tikz-utils.tex <==
%

\usepackage{tikz}


\usetikzlibrary{positioning,
  intersections,
  hobby,
  patterns,
  calc,
  decorations.pathmorphing,
  decorations.markings,
  shadows,
  shapes,
  cd,
  decorations.markings,
  positioning,
  arrows.meta,
  shapes,
  calc,
  fit,
  quotes,
backgrounds}

\usepackage{tikzpagenodes}

%

\tikzcdset{arrow style=tikz}
\tikzstyle{arrowmorphismstyle} = [-{Triangle[width=3.5pt,length=3.5pt]},draw=morphisms]
\tikzstyle{arrownorphismstyle} = [-{Triangle[width=3.5pt,length=3.5pt]},dashed, draw=norphisms]
\tikzstyle{arrowmorphismstylemapsto} = [|-{Triangle[width=3.5pt,length=3.5pt]},draw=morphisms]
\tikzstyle{arrowfunctorstyle} = [-{Triangle[width=3.5pt,length=3.5pt]},draw=functors]
\tikzstyle{block} = [draw=morphisms, rectangle, minimum height=2em, minimum width=3em, thick]
\tikzstyle{blockgroup} = [draw=morphisms, rectangle, minimum height=2em, minimum width=3em, dotted, thick]
\tikzstyle{resblock} = [draw=red, rectangle, minimum height=2em, minimum width=3em, thick]
\tikzstyle{compblock} = [draw=blue, rectangle, minimum height=2em, minimum width=3em, thick]
\tikzstyle{effblock} = [draw=black, rectangle, minimum height=2em, minimum width=3em, thick]
\tikzstyle{tupblock} = [draw=morphisms, rectangle, minimum height=2em, minimum width=3em, thick]
\tikzstyle{styleobjects} = [draw=objects, thick]
\tikzstyle{morblock} = [draw=morphisms, rectangle, minimum height=2em, minimum width=3em, thick, rounded corners=2]
\tikzstyle{norblock} = [draw=norphisms, rectangle, minimum height=2em, minimum width=3em, thick, rounded corners=2]

\tikzstyle{blockk} = [draw, rectangle, minimum height=2.5em, minimum width=3.5em]
\tikzstyle{block1} = [draw, rectangle, minimum height=1.5em, minimum width=2.5em]
\tikzstyle{blockDyn} = [draw, rectangle, minimum height=2.5em, minimum width=3.5em, align=center, inner sep=10pt, thick, fill=white, copy shadow={draw=black,fill=black,opacity=1,shadow xshift=0.5ex,shadow yshift=-0.5ex}]
\tikzstyle{blockAlg} = [draw, rectangle, minimum height=1.5em, minimum width=2.5em, align=center, inner sep=10pt, thick]
\tikzstyle{sum} = [draw,circle]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
%

%

%
%
%

%
\tikzcdset{every label/.append style={font=\normalsize}}
\def\preceqSize{10pt}
\newcommand{\hasselinewidth}{2mm}


\tikzset{fcname/.store in =\fcname, fcname={}}
\tikzset{funame/.store in =\funame, funame={}}
\tikzset{rcname/.store in =\rcname, rcname={}}
\tikzset{runame/.store in =\runame, runame={}}
\tikzset{whereres/.store in =\whereres, whereres=0.5}
\tikzset{wherefun/.store in =\wherefun, wherefun=0.5}
\tikzset{relres/.store in =\relres, relres={right}}
\tikzset{relfun/.store in =\relfun, relfun={left}}
\tikzset{posres/.store in =\posres, posres=0.95}
\tikzset{posfun/.store in =\posfun, posfun=0.95}
\tikzset{loos/.store in =\loos, loos=2}
\tikzset{feedback/.store in =\feedback, feedback=0}
\tikzset{
  DP/.style={%
    %
    label/.style={
      font=\everymath\expandafter{\the\everymath\scriptstyle},
      inner sep=5pt,
      node distance=2pt and -2pt},
    semithick,
    node distance=1 and 1,
    rconn/.style={color=white,opacity=0.0,postaction={decorate}, shorten <=3.2pt, shorten >= 0.8,
    decoration={markings,
    mark= at position 0 with {
      \coordinate (a);
    },
    mark=at position .5 with
        {
        \ifthenelse{\equal{\feedback}{1}}{\def\angleOut{-90}\def\angleIn{-90}}{\def\angleOut{0}\def\angleIn{180}}
        \coordinate (b);
        \draw[dashed,\dpred,opacity=1.0] (a) to[out=\angleOut,in=\angleIn,looseness=\loos]
        node[pos=\posres,\relres=\whereres mm,\dpred,opacity=1,fill=white,inner sep=1pt,outer sep=1pt]{\rcname} (b);
      },
      mark= at position 1 with
        {
        \ifthenelse{\equal{\feedback}{1}}{\def\angleOut{0}\def\angleIn{0}}{\def\angleOut{180}\def\angleIn{0}}
        \ifthenelse{\equal{\feedback}{1}}{\def\symbol{\succeq}}{\def\symbol{\preceq}}
        \coordinate (c);
        \draw[\dpgreen,opacity=1.0] (c) to[out=\angleOut,in=\angleIn,looseness=\loos]
        node[pos=\posfun,\relfun=\wherefun mm,\dpgreen,opacity=1,fill=white,inner sep=1pt,outer sep=1pt]{\fcname} (b){}; %
        \node[draw,circle,inner sep=0.5pt,color=black,fill=white,opacity=1.0,line width=0.2mm] at (b) (nodepreceq) {$\symbol$};
      }
    }},
    runconn/.style={color=\dpred,dashed,postaction={decorate},
    decoration={markings,
    mark= at position 1 with {
      \coordinate (a);
      \draw[\dpred,opacity=1.0,dashed] ($(a)+(0.05,0)$) --++ (0.5,0) node[\relres,pos=\posres]{\runame};}
    }
    },
    funconn/.style={color=white,postaction={decorate},
    decoration={markings,
    mark= at position 0 with {
      \coordinate (a);
      \draw[\dpgreen] ($(a)+(-0.05,0)$) -- ($(a)+(-0.5,0)$) node[\relfun,pos=\posfun]{\funame};}
    }
    },
    execute at begin picture={\tikzset{
      x=\dpx, y=\dpy,
      every fit/.style={inner xsep=\dpx, inner ysep=\dpy}}}
  },
  dpx/.store in=\dpx,
  dpx = 1.5cm,
  dpy/.store in=\dpy,
  dpy = 1.5ex,
  dp port sep/.store in=\dpportsep,
  dp port sep=2,
  dp port length/.store in=\dpportlen,
  dp port length=4pt,
  dp min width/.store in=\dpminwidth,
  dp min width=0.5cm,
  dp rounded corners/.store in=\dpcorners,
  dp rounded corners=2pt,
  dp small/.style={dp port sep=1, dp port length=2.5pt, dpx=.4cm, dp min width=.4cm, dpy=.7ex},
  dp/.code 2 args={%
    %
    %
    \pgfmathsetlengthmacro{\dpheight}{\dpportsep * (max(#1,#2)) * \dpy}
    \pgfkeysalso{draw,%
      minimum width=\dpminwidth,%
      minimum height=\dpheight,%
    %
      outer sep=0pt,%
      inner sep=5pt,%
      rounded corners=\dpcorners,
      thick,
      prefix after command={\pgfextra{\let\fixname\tikzlastnode}},
      append after command={\pgfextra{\draw
      \ifnum #1=0{} \else foreach \i in {1,...,#1} {
        ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(0,0) node[solid,left,circle,color=\dpgreen,draw,fill=\dpgreen,scale=0.3] {} coordinate (\fixname_fun\i) -- +(0,0) coordinate (\fixname_fun\i')}\fi %
      \ifnum #2=0{} \else foreach \i in {1,...,#2} {
        ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(0,0) coordinate (\fixname_res\i') -- +(0,0) node[solid,right,circle,color=\dpred,draw,fill=\dpred,scale=0.3] {} coordinate (\fixname_res\i)}\fi;
      }}}
  },
  dp name/.style={append after command={\pgfextra{\node[label=center,inner sep=2pt,fill=white] at (\fixname) {#1};}}}
}

\tikzset{
  oriented WD/.style={%
    every to/.style={out=0,in=180,draw},
    label/.style={
      font=\everymath\expandafter{\the\everymath\scriptstyle},
      inner sep=0pt,
      node distance=2pt and -2pt},
    semithick,
    node distance=1 and 1,
    decoration={markings, mark=at position .5 with {\arrow{stealth};}},
    ar/.style={postaction={decorate}},
    execute at begin picture={\tikzset{
      x=\bbx, y=\bby,
      every fit/.style={inner xsep=\bbx, inner ysep=\bby}}}
  },
  bbx/.store in=\bbx,
  bbx = 1.5cm,
  bby/.store in=\bby,
  bby = 1.75ex,
  bb port sep/.store in=\bbportsep,
  bb port sep=2,
%
%
  bb port length/.store in=\bbportlen,
  bb port length=4pt,
  bb min width/.store in=\bbminwidth,
  bb min width=1cm,
  bb rounded corners/.store in=\bbcorners,
  bb rounded corners=2pt,
  bb small/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, bby=.7ex},
  bb/.code 2 args={%
    \pgfmathsetlengthmacro{\bbheight}{\bbportsep * (max(#1,#2)+1) * \bby}
    \pgfkeysalso{draw,minimum height=\bbheight,minimum width=\bbminwidth,outer sep=0pt,
      rounded corners=\bbcorners,thick,
      prefix after command={\pgfextra{\let\fixname\tikzlastnode}},
      append after command={\pgfextra{\draw
      \ifnum #1=0{} \else foreach \i in {1,...,#1} {
        ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(-\bbportlen,0) coordinate (\fixname_in\i) -- +(\bbportlen,0) coordinate (\fixname_in\i')}\fi %
      \ifnum #2=0{} \else foreach \i in {1,...,#2} {
        ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbportlen,0) coordinate (\fixname_out\i') -- +(\bbportlen,0) coordinate (\fixname_out\i)}\fi;
      }}}
  },
  bb name/.style={append after command={\pgfextra{\node[anchor=north] at (\fixname.north) {#1};}}}
}

\tikzset{
  tick/.style={postaction={
    decorate,
    decoration={markings, mark=at position 0.5 with {\draw[-] (0,.4ex) -- (0,-.4ex);}}}
  }
}

%
\newcommand{\vmiddle}[1]{\raisebox{-0.5\height}{#1}}
%

\newcommand{\middlesag}[1]{%
  \vmiddle{\saginclude{#1}}
}
\newcommand{\includesag}[1]{%
%
%
%
  \saginclude{#1}
}

\newcommand{\saginclude}[1]{%
    \def\pdffile{\sagdir/\detokenize{#1}.pdf}%
    \def\srcfile{\sagdir/\detokenize{#1}.tikz}%
    \ifbool{cachepdf}{%
        \IfFileExists{\pdffile}{%
            \Filemodcmp{\pdffile}{\srcfile}{%
                \includegraphics[scale=1]{\pdffile}%
            }{%
                \PackageWarning{ACT4E}{TikZ file is more recent than outdated pdf cache \pdffile}%
                \input{\srcfile}%
            }%
        }{\input{\srcfile}}%
    }{%
        \input{\srcfile}%
    }%
}

\newcommand{\equationsag}[2]{%
%
%
%
\begin{equation}%
  \middlesag{#1}%
  \ifemptyarg{#2}{%
 \PackageError{ACT4E}{Empty label argument}{You passed empty label}
}{\label{#2}}
\end{equation}%
}


%
%
%
%
%

\newcommand{\blfootnote}[1]{\footnote{#1}}
\usetikzlibrary{calc}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\newlength{\brickwidth}
\newlength{\brickheight}
\newlength{\brickdia}
\newlength{\brickdiaheight}
\newlength{\brickmultipliedx}
\newlength{\brickmultipliedy}
\newlength{\halfbrickwidth}
\setlength{\brickheight}{9.6mm}
\setlength{\brickwidth}{8mm}
\setlength{\brickdia}{2.8mm}
\setlength{\brickdiaheight}{1mm}
\setlength{\halfbrickwidth}{0.5\brickwidth}

\newcommand{\startpos}[3]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)$)}
\newcommand{\startposcustom}[4]{($(0,#3*#4)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)$)}

\newcommand{\startposplusheight}[3]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(0mm,\brickheight)$)}

\newcommand{\startposplusheightcustom}[4]{($(0,#3*#4)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(0mm,#4)$)}

\newcommand{\pinposone}[5]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(-0.05\brickwidth,1.35\brickheight)$)}
%
%
\newcommand{\pinposonecustom}[6]{($(0,#3*#6)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(-0.05\brickwidth,1.35*#6)$)}


\newcommand{\pinpostwo}[5]{($(0,#3\brickheight)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(0.3\brickwidth,1.35\brickheight)$)}

\newcommand{\pinpostwocustom}[6]{($(0,#3*#6)+(7:#1\brickwidth)+(138:#2\halfbrickwidth)+(7:#4*\brickwidth)+(138:#5*\halfbrickwidth)+(-0.6\brickwidth,-\halfbrickwidth)+(0.3\brickwidth,1.35*#6)$)}

\newcommand{\brick}[6]{%
  \setlength{\brickmultipliedx}{#1\brickwidth}
  \setlength{\brickmultipliedy}{#2\brickwidth}
  \filldraw[fill=#3,draw=black,thick] \startpos{#4}{#5}{#6} -- ++(7:\brickmultipliedx) -- ++(0mm,\brickheight) -- ++(138:0.5\brickmultipliedy) -- ++(187:\brickmultipliedx) -- ++(0mm,-\brickheight) -- cycle;
  \draw[black,thick] \startpos{#4}{#5}{#6} -- ++(0mm,\brickheight) -- ++(138:0.5\brickmultipliedy);
  \draw[black,thick] \startposplusheight{#4}{#5}{#6} -- ++(7:\brickmultipliedx);
  \foreach \i in {1,...,#1} {
    \foreach \j in {1,...,#2} {
      \pin{\pinposone{#4}{#5}{#6}{\i}{\j}}{\pinpostwo{#4}{#5}{#6}{\i}{\j}}{#3}
    }
  }
}

\newcommand{\brickcustom}[7]{%

  \setlength{\brickmultipliedx}{#1\brickwidth}
  \setlength{\brickmultipliedy}{#2\brickwidth}
  \filldraw[fill=#3,draw=black,thick, rounded corners=0] \startposcustom{#4}{#5}{#6}{#7\brickheight} -- ++(7:\brickmultipliedx) -- ++(0mm,#7\brickheight) -- ++(138:0.5\brickmultipliedy) -- ++(187:\brickmultipliedx) -- ++(0mm,-#7\brickheight) -- cycle;
  \draw[black,thick, rounded corners=0] \startposcustom{#4}{#5}{#6}{#7\brickheight} -- ++(0mm,#7\brickheight) -- ++(138:0.5\brickmultipliedy);
  \draw[black,thick,rounded corners=0] \startposplusheightcustom{#4}{#5}{#6}{#7\brickheight} -- ++(7:\brickmultipliedx);
  \pgfmathsetmacro\weight{1/#7}
  \foreach \i in {1,...,#1} {
    \foreach \j in {1,...,#2} {
%
%
%
      \pincustom{\pinposonecustom{#4+0.075*\weight}{#5+0.4+0.2*\weight}{#6}{\i}{\j}{#7\brickheight}}{\pinpostwocustom{#4+0.075*\weight}{#5+0.2*\weight}{#6}{\i}{\j}{#7\brickheight}}{#3}{#7\brickheight}
    }
  }
}

\newcommand{\brickcustomtr}[7]{%

  \setlength{\brickmultipliedx}{#1\brickwidth}
  \setlength{\brickmultipliedy}{#2\brickwidth}
  \filldraw[fill=none,draw=none,thick, rounded corners=0] \startposcustom{#4}{#5}{#6}{#7\brickheight} -- ++(7:\brickmultipliedx) -- ++(0mm,#7\brickheight) -- ++(138:0.5\brickmultipliedy) -- ++(187:\brickmultipliedx) -- ++(0mm,-#7\brickheight) -- cycle;
  \draw[draw=none,thick, rounded corners=0] \startposcustom{#4}{#5}{#6}{#7\brickheight} -- ++(0mm,#7\brickheight) -- ++(138:0.5\brickmultipliedy);
  \draw[draw=none,thick,rounded corners=0] \startposplusheightcustom{#4}{#5}{#6}{#7\brickheight} -- ++(7:\brickmultipliedx);
  \pgfmathsetmacro\weight{1/#7}
  \foreach \i in {1,...,#1} {
    \foreach \j in {1,...,#2} {
%
%
%
      \pincustomtr{\pinposonecustom{#4+0.075*\weight}{#5+0.4+0.2*\weight}{#6}{\i}{\j}{#7\brickheight}}{\pinpostwocustom{#4+0.075*\weight}{#5+0.2*\weight}{#6}{\i}{\j}{#7\brickheight}}{#3}{#7\brickheight}
    }
  }
}

\newcommand{\pin}[3]{%
  \filldraw[fill=#3,draw=black,thick] #1 -- ++(0mm,-1.6\brickdiaheight) .. controls +(\brickdia,-0.1\brickheight) .. ++(2\brickdia,0mm) -- ++(0mm,1.6\brickdiaheight) -- cycle;
  \filldraw[fill=#3,draw=black,thick] #2 ellipse[x radius=\brickdia, y radius=\brickdiaheight];
}

\newcommand{\pincustom}[4]{%
  \filldraw[fill=#3,draw=black,thick, rounded corners=0] #1 -- ++(0mm,-1.6\brickdiaheight) .. controls +(\brickdia,-0.1*#4) .. ++(2\brickdia,0mm) -- ++(0mm,1.6\brickdiaheight) -- cycle;
  \filldraw[fill=#3,draw=black,thick, rounded corners=0] #2 ellipse[x radius=\brickdia, y radius=\brickdiaheight];
}

\newcommand{\pincustomtr}[4]{%
  \filldraw[fill=none,draw=none,thick, rounded corners=0] #1 -- ++(0mm,-1.6\brickdiaheight) .. controls +(\brickdia,-0.1*#4) .. ++(2\brickdia,0mm) -- ++(0mm,1.6\brickdiaheight) -- cycle;
  \filldraw[fill=none, draw=none,thick, rounded corners=0] #2 ellipse[x radius=\brickdia, y radius=\brickdiaheight];
}


%
\newlength{\hatchspread}
\newlength{\hatchthickness}
\newlength{\hatchshift}
\newcommand{\hatchcolor}{}
%
\tikzset{hatchspread/.code={\setlength{\hatchspread}{#1}},
  hatchthickness/.code={\setlength{\hatchthickness}{#1}},
  hatchshift/.code={\setlength{\hatchshift}{#1}},%
  hatchcolor/.code={\renewcommand{\hatchcolor}{#1}}}
%
\tikzset{hatchspread=3pt,
  hatchthickness=0.4pt,
  hatchshift=0pt,%
  hatchcolor=black}
%
\pgfdeclarepatternformonly[\hatchspread,\hatchthickness,\hatchshift,\hatchcolor]%
{custom north west lines}%
{\pgfqpoint{\dimexpr-2\hatchthickness}{\dimexpr-2\hatchthickness}}%
{\pgfqpoint{\dimexpr\hatchspread+2\hatchthickness}{\dimexpr\hatchspread+2\hatchthickness}}%
{\pgfqpoint{\dimexpr\hatchspread}{\dimexpr\hatchspread}}%
{%
  \pgfsetlinewidth{\hatchthickness}
  \pgfpathmoveto{\pgfqpoint{0pt}{\dimexpr\hatchspread+\hatchshift}}
  \pgfpathlineto{\pgfqpoint{\dimexpr\hatchspread+0.15pt+\hatchshift}{-0.15pt}}
  \ifdim \hatchshift > 0pt
  \pgfpathmoveto{\pgfqpoint{0pt}{\hatchshift}}
  \pgfpathlineto{\pgfqpoint{\dimexpr0.15pt+\hatchshift}{-0.15pt}}
  \fi
  \pgfsetstrokecolor{\hatchcolor}
%
  \pgfusepath{stroke}
}



\newcommand{\stain}[1]{
\scalebox{0.08}{
\begin{tikzpicture}[use Hobby shortcut,closed=true]
      %
      %
        %
      \draw[fill=#1,line width=6,rounded corners=0](-2.5,-0.5).. (-3.5,0).. (-2.5,0.5).. (-3,1).. (-2,1.5).. (-2,3).. (-1,2.5).. (1,4.5).. (2.5,3).. (3,3.5).. (3.5,3).. (3,2).. (4.5,2).. (4.5,0).. (3,1).. (2.5,-0.5).. (3.5,-1.5).. (1.5,-1).. (0.5,-2).. (-2,-2.5).. (-1.5,-1).. (-2.5,-1.5).. (-2.5,-0.5);
\end{tikzpicture}}}

\newcommand{\vstain}[1]{\vmiddle{\stain{#1}}}
\newcommand{\vstainfilled}[1]{\vmiddle{\stainfilled{#1}}}

\newcommand{\stainfilled}{
\scalebox{0.08}{
\begin{tikzpicture}[use Hobby shortcut,closed=true]
      \draw[pattern=custom north west lines,line width=6,hatchspread=3pt,hatchthickness=1pt,draw=black, rounded corners=0](-2.5,-0.5).. (-3.5,0).. (-2.5,0.5).. (-3,1).. (-2,1.5).. (-2,3).. (-1,2.5).. (1,4.5).. (2.5,3).. (3,3.5).. (3.5,3).. (3,2).. (4.5,2).. (4.5,0).. (3,1).. (2.5,-0.5).. (3.5,-1.5).. (1.5,-1).. (0.5,-2).. (-2,-2.5).. (-1.5,-1).. (-2.5,-1.5).. (-2.5,-0.5);
\end{tikzpicture}
}
}
%
%
%
%
%
%
%

\newcommand{\figplug}[1]{
 #1~\includegraphics[height=2cm,angle=-90,origin=c]{plugs/#1-button}
}

\newcommand{\comma}[2]{
\begin{tikzpicture}
\node at (0,0) {#1 \Huge{,}#2};
\end{tikzpicture}}


\newcommand{\cordG}[1]{%
  \raisebox{-2.6pt}{\includegraphics[width=4mm]{socket}}%
  \hspace{-1.3mm}%
  -#1-%
  \hspace{-1.3mm}\raisebox{-2.2pt}{\includegraphics[width=4mm]{plug}}}
%

\newcommand{\cord}[3]{
 \begin{tikzpicture}
 \node (flaga) at (0,0) {#1};
 \node[right=0.02cm of flaga] (sock) {\includegraphics[width=4mm]{socket}};
 \node[right=0.02cm of sock](lab) {$#2$};
  \draw ($(sock.east)+(-0.125,0)$) --  ($(lab.west)-(-0.05,0)$) {};
 \node[right=0.02cm of lab](plug){ \includegraphics[width=4mm]{plug}};
 \draw ($(lab.east)+(-0.075,0)$) --  ($(plug.west)+(0.125,0)$) {};
 \node[right=0.02cm of plug] {#3};
 \end{tikzpicture}
}

\newcommand{\homtemplate}[6]{
\begin{tikzpicture}
\node[block,draw=morphisms] (one) at (0,0) {$#1$};
\node[block, right=0.5cm of one, dashed, fill=yellow] (two) {};
\node[block, right=0.5cm of two,draw=morphisms] (three) {$#2$};
\draw[-, thick] (one.east) -- node[pos=0.5,above] {$#3$}(two.west) {};
\draw[-, thick] (two.east) -- node[pos=0.5,above] {$#4$}(three.west) {};
\draw[-, thick] ($(one.west)+(-0.5,0)$) -- node[pos=0.5,above] {$#5$}(one.west) {};
\draw[-, thick] (three.east) -- node[pos=0.5,above] {$#6$}($(three.east)+(0.5,0)$) {};
\end{tikzpicture}
}

%

%
\newcommand{\TypeIrish}{\includegraphics[height=2mm]{flag-ireland}}
\newcommand{\TypeSwiss}{\includegraphics[height=2mm]{flag-swiss}}
\newcommand{\TypeFrench}{\includegraphics[height=2mm]{flag-france}}
\newcommand{\TypeItalian}{\includegraphics[height=2mm]{flag-italy}}
\newcommand{\TypeUSA}{\includegraphics[height=2mm]{flag-usa}}
\newcommand{\TypeChinese}{\includegraphics[height=2mm]{flag-china}}


\newcommand{\dashedbox}[1]{
%
%
\begin{tikzpicture}
\draw[#1, ultra thick, rounded corners=0] (-0.25,-0.25) rectangle (0.5,0.5){};
\end{tikzpicture}%
%
}

\newcommand{\dashedboxfilled}[2]{
%
%
\begin{tikzpicture}
\draw[#1, ultra thick, rounded corners=0] (-0.25,-0.25) rectangle node[pos=0.5, black]{#2} (0.5,0.5){};
\end{tikzpicture}%
%
}

\newcommand{\dashedboxinv}[2]{
%
\begin{tikzpicture}
\draw[white, text=#2, ultra thick,dashed, rounded corners=0] (-0.25,-0.25) rectangle (0.5,0.5) node[pos=0.5, text=#2]{\textcolor{#2}{#1}};
\end{tikzpicture}%
%
}


\newcommand{\roundbox}[1]{
\begin{tikzpicture}
\draw[#1, ultra thick,dashed] (-0.25,-0.25) circle (0.35);
\end{tikzpicture}
}

\newcommand{\filledbox}[2]{
\begin{tikzpicture}
\draw[black, ultra thick,fill=#1] (-0.5,-0.275*#2) rectangle (1.5,0.55*#2){};
\end{tikzpicture}
}

\newcommand{\coloredbox}[1]{
\begin{tikzpicture}
\draw[#1, ultra thick,fill=#1] (-0.25,-0.25) rectangle (1, 0.5);
\end{tikzpicture}
}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%
%
%
%
%
%
%
%
\newcommand{\rope}[7]{
\begin{tikzpicture}[n/.style={circle,draw,minimum size=2mm,inner sep=0, fill=#1}, remember picture]
\ifthenelse{\lengthtest{#5 pt=0 pt} \AND \lengthtest{#6 pt=1 pt}}
{\draw[ultra thick, #1] (0,0) -- node[pos=#5, #1,n]{} node[pos=#6,n] {} node[pos=0.5, above, black]{#7} (#3,#4){};}
{\draw[ultra thick, #1] (#5*#3,#5*#4) -- node[pos=0, #1,n,overlay]{} node[pos=1, #1,n] {} node[pos=0.5, above, black]{#7} (#6*#3,#6*#4){};
\begin{pgfonlayer}{background}
\draw[ultra thick, #2] (0,0)--(#5*#3,#5*#4){};
\draw[ultra thick, #2] (#6*#3,#6*#4)--(#3,#4){};
\end{pgfonlayer}}
\end{tikzpicture}}



\newcommand{\northenasymb}{%
\mathbin{\begin{tikzpicture}[n/.style={circle,draw,minimum size=0.8mm,inner sep=0, fill=black}]
%
\node[n] at (0.125,0.05) {};
\node at (0.1,0.1){};
\draw[thick](0,0.05)--(0.25,0.05){};
\end{tikzpicture}}}

\newcommand{\northenbsymb}{%
\mathbin{\begin{tikzpicture}[n/.style={circle,draw,minimum size=0.8mm,inner sep=0, fill=black}]
\node[n] at (0,0.05) {};
\node[n] at (0.2,0.05) {};
\node at (0.1,0.1){};
\draw[thick](0,0.05)--(0.2,0.05){};
\end{tikzpicture}}}

\newcommand{\northena}[2]{{#1 \northenasymb #2}}
\newcommand{\northenb}[2]{{#1 \northenbsymb  #2}}




%
%
%
\newcommand{\ropeknot}[6]{
\begin{tikzpicture}[n/.style={circle,draw,minimum size=2mm,inner sep=0, fill=#1}, m/.style={circle,draw,minimum size=1.5mm,inner sep=0, fill=none}, remember picture]
  \draw[#6,thick, fill=none] ($(#4,#5)-(0,0.25)$) -- node[pos=0, #6,m]{} node[pos=1, #6,m]{} ($(#4,#5)+(0,0.25)$){};
\draw[ultra thick, #1] (0,0) -- node[pos=0, #1,n]{} node[pos=1, #1,n]{} (#2,#3){};
\end{tikzpicture}}


\usepackage{forest}

\newcommand{\dirtree}[1]{%
    \begin{forest}
      for tree={
        font=\ttfamily,
        grow'=0,
        child anchor=west,
        parent anchor=south,
        anchor=west,
        calign=first,
        edge path={
          \noexpand\path [draw, \forestoption{edge}]
          (!u.south west) +(4.5pt,0) |- node[fill,inner sep=1.25pt] {} (.child anchor)\forestoption{edge label};
        },
        before typesetting nodes={
          if n=1
            {insert before={[,phantom]}}
            {}
        },
        fit=band,
        before computing xy={l=15pt},
      }
    #1
    \end{forest}
}

%
%
%
%
\definecolor{cblue}{rgb}{0.3,0.3,1.0}
\definecolor{cred}{rgb}{1.0,0.1,0.1}

\definecolor{cwhite}{rgb}{0.95,0.95,0.97}
\definecolor{funbox}{rgb}{0.92,1,0.9}
\definecolor{resbox}{rgb}{1,0.74,0.75}
\definecolor{impbox}{rgb}{1,0.92,0.85}

\newcommand{\legob}[1]{%
\adjustbox{scale=0.4}{\includesag{intro-lego-#1}}%
}

\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes.symbols}

\newcommand{\shadowbox}[1]{
\begin{tikzpicture}
\node[draw=gray,shade,
      top color=white,
      bottom color=white,
      rounded corners=6pt,
      blur shadow={shadow blur steps=6}
    ] {#1};
\end{tikzpicture}}

\definecolor{red1}{rgb}{0.30,0,0}
\definecolor{red2}{rgb}{0.60,0,0}
\definecolor{red3}{rgb}{0.90,0,0}
\definecolor{my-cyan}{cmyk}{1,0,0,0}
\definecolor{my-magenta}{cmyk}{0,1,0,0}
\definecolor{my-yellow}{cmyk}{0,0,1,0}
%


\newcommand{\funbox}[3]{
\begin{tikzpicture}
\node[draw=funbox,
      fill=funbox,
      minimum height =2cm,
minimum width =2cm,
      rounded corners=6pt] at (#1,#2) {#3};
\end{tikzpicture}}

\newcommand{\resbox}[3]{
\begin{tikzpicture}
\node[draw=resbox,
      fill=resbox,
      minimum height =2cm,
minimum width =2cm,
      rounded corners=6pt] at (#1,#2) {#3};
\end{tikzpicture}}

\newcommand{\impbox}[3]{
\begin{tikzpicture}
\node[draw=impbox,
      fill=impbox,
      minimum height =2cm,
minimum width =2cm,
      rounded corners=6pt] at (#1,#2) {#3};
\end{tikzpicture}}

\newcommand{\boxset}[1]{
\begin{tikzpicture}
\node[draw=setcolor,
      fill=setcolor,
      rounded corners] at (0,0) {#1};
\end{tikzpicture}}

\tikzcdset{
    setcd/.style={
        every matrix/.append style={
            draw=setcolorbord,
            fill=setcolor,
            rounded corners,
            inner sep=1pt,
            #1
        },
    },
}

\tikzcdset{
    posetcd/.style={
        every matrix/.append style={
            draw=posetcolorbord,
            fill=posetcolor,
            rounded corners,
            inner sep=1pt,
            #1
        },
    },
}

\tikzcdset{
    catcd/.style={
        every matrix/.append style={
            draw=catcolor,
            fill=catcolor,
            rounded corners,
            inner sep=4pt,
            #1
        },
    },
}

\tikzcdset{
    graphcd/.style={
        every matrix/.append style={
            draw=graphcolorbord,
            fill=graphcolor,
            rounded corners,
            inner sep=4pt,
            #1
        },
    },
}

%
\newcommand{\labelobleft}[2]{
    \node[left=0mm of #1.south west, anchor=south east] {#2};
}
%
\newcommand{\labelobtop}[2]{
    \node[above left=0mm of #1.north west, anchor=south west] {#2};
}

\newcommand{\arrowbgcolor}{white}

